The pop song generator: designing an online course to teach collaborative, creative AI

This article describes and evaluates a new online AI-creativity course. The course is based around three near-state-of-the-art AI models combined into a pop song generating system. A fine-tuned GPT-2 model writes lyrics, Music-VAE composes musical scores and instrumentation and Diffsinger synthesises a singing voice. We explain the decisions made in designing the course which is based on Piagetian, constructivist 'learning-by-doing'. We present details of the five-week course design with learning objectives, technical concepts, and creative and technical activities. We explain how we overcame technical challenges to build a complete pop song generator system, consisting of Python scripts, pre-trained models, and Javascript code that runs in a dockerised Linux container via a web-based IDE. A quantitative analysis of student activity provides evidence on engagement and a benchmark for future improvements. A qualitative analysis of a workshop with experts validated the overall course design, it suggested the need for a stronger creative brief and ethical and legal content.

==> RemovedSections.tex <==
Original abstract:

Explainable AI seeks to make the underlying algorithmic manoeuvres of AI systems more transparent so that individuals and societies can develop greater trust in their outputs.
Creative collaboration with an AI systems involves dynamic interaction, where explanations that allow us to better understand how to collaborate effectively are sought in real-time as the collaboration unfolds, as well as after the interaction. We present a methodological approach to study explainability in Human/AI music improvisation. We investigate how ongoing information between musicians and an AI system can improve collaboration when improvising as a duo. Participants improvised with an AI sequencer, annotating performances when they would have liked to better understand what the system is doing, or be able to communicate their musical intentions with the system. Through thematic analysis, we identify general design considerations for the development of creative AI systems in improvised performance settings.


Mark's abstract: 
For over a decade the majority of AI research exploring creativity has tended to focus on qualities of the output or outcome of the AI system. 
%
This system is either thought of as the lone heroic creating music, art and poems independently of human intervention or in providing a collaboration with a human user. %
Typically - so the argument goes - we can find creativity in the AI system by exploring properties of the output: originality, value and significance are typical examples.  
%
In this paper we adopt a different approach and explore the degree to which an AI improvising system can challenge, provoke and stimulate new kinds of human creative musicianship. 
% 
In fact we are interested in a very specific question: what are the ways in which the human and AI can signal to each what state or intention they are currently they are in. 
%
It is our thesis that even being able to explain to the machine what the musicians intention or desire is, and for the machine to signal what algorithmic choices it is making opens up new possibilities for creative musicianship in practice and performance. 
%
One of the great challenges of AI is to devise systems that can challenge, stimulate and provoke human creativity in new kinds of ways
%
In this paper we specifically lay the theoretical, practical and experimental foundations for understand the role of explainabilty in human/AI interaction. 
%
This approach promises new ways of understanding the opportunity for AI to stimulate, challenge and provoke new kinds of creativity in their artistic endeavours. 



\begin{figure} 
    \centering
    \begin{subfigure}{0.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{WordCloud_AnnotationFiles_cropped.png}
        \caption{Word Cloud from participants' annotations in \textit{Music Circle}.}
        \Description{Word Frequency Cloud from participants' annotations in \textit{Music Circle}.}
        \label{fig:wordcloud_annotations}
    \end{subfigure}%
    \begin{subfigure}{0.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{WordCloud_InterviewFiles_cropped.png}
        \caption{Word Cloud from participants' interview transcriptions.}
        \Description{Word Frequency Cloud from participants' interview transcriptions.}
        \label{fig:wordcloud_interviews}
    \end{subfigure}
    \caption{Word Frequency Clouds from (a) participant annotations in \textit{Music Circle} and (b) participant interviews. The size of each word represents it's frequency.}
    \Description{Two word clouds are shown depicting scattered words of differing sizes. The left word cloud represents participants' annotations in \textit{Music Circle} and the right word cloud represents represents participants' interviews. The size of each word represents it's frequency.}
    \label{fig:wordclouds}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{MusicCircleScreenShot_AllInOne.png}
    \caption{\textit{\textit{Music Circle}} annotation platform showing participant annotations along a timeline of their collaborative improvisation with the system.}
    \Description{\textit{Music Circle} music annotation platform showing four audio wave forms stacked vertically from top to bottom. In each wave from a small section of the audio recording has been highlighted and a comment is shown.}
    \label{fig:MusicCircle}
\end{figure}


\begin{table}[htbp]
\centering
\begin{tabular}{c|c|c|l}
Participant & Gender & Age Range & Musical Background \\\hline
P1 & M & 20-30 & Advanced knowledge of music theory \\
P2 & M & 20-30 & Advanced knowledge of music theory \\
P3 & M & 40-50 & Basic knowledge of music theory \\
P4 & M & 30-40 & Professional musician \\
P5 & M & 20-30 & Advanced knowledge of music theory \\
\end{tabular}
\caption{\label{tab:participants}Table of participant demographics.}
\end{table}


\begin{table}[htbp]
\centering
\begin{tabular}{|l|l|l|}
\hline
%\multicolumn{1}{|c}{\textbf{Theme}} & \multicolumn{1}{|c}{\textbf{Codes}} &\multicolumn{1}{|c|}{\textbf{Code references (\% of Theme Total)}}\\
\textbf{Theme} & \textbf{Codes} & \textbf{Code references (\% of Theme Total)}\\
\hline
\multirow{ 3}{*}{Human Interaction}         & Musical interaction & \mybar{5.8} 58\% \\ 
                                            & Physical interaction & \mybar{3.1} 31\%\\
                                            & Past experiences & \mybar{1.1} 11\%\\
\hline
\multirow{ 3}{*}{Understanding the system}  & Expected musical knowledge & \mybar{6.8} 68\% \\ 
                                            & Experimenting & \mybar{2.9} 29\%\\
                                            & Understanding patterns & \mybar{0.3} 3\%\\
\hline
\multirow{ 3}{*}{Structured Improvisation}  & Leading and accompanying & \mybar{6.7} 67\% \\ 
                                            & Pre-performance baseline & \mybar{1.8} 18\%\\
                                            & Stages during performance & \mybar{1.5} 15\%\\
\hline
\multirow{ 5}{*}{Explicit Communication}    & Signal change to the system & \mybar{3.9} 39\% \\ 
                                            & Signal good interaction & \mybar{2.2} 22\%\\
                                            & Signal unwanted interaction & \mybar{1.9} 19\% \\
                                            & Signal end of performance & \mybar{1.3} 13\%\\
                                            & System signalling to user & \mybar{0.7} 7\%\\
\hline
\multirow{ 2}{*}{Implicit Communication}    & Musical cue & \mybar{6.8} 68\%\\ 
                                            & Physical cue & \mybar{3.2} 32\%\\
\hline
\end{tabular}
\caption{Themes and codes identified through thematic analysis of participant interviews and annotations.}
\label{tab:themes}
\end{table}


\Section{Methodology}
%\vspace{-10cm}
At the beginning of the session, participants were first asked to familiarise themselves with the system for at least five minutes. Participants were then asked to collaborate with the system to create and record an improvised performance. The participants were asked to sustain a performance for at least five minutes and were also asked to carry out this task for at least two sessions in order to assess multiple collaborations with the system. 

Audio and MIDI recordings of the improvisational piece were automatically saved and uploaded to \textit{Music Circle}. Participants were then asked to annotate any part of the audio recording by placing comments along the timeline. In \textit{Music Circle} the participant first identifies a segment of the performance and then annotates it using one of the following tags:

\begin{small}
\begin{description}
\item {\bf {\em intention\_system}}: I would like to have known what the system was doing here.
\item {\bf {\em intention\_mine}}: I would have liked to let the system know what I was doing here.
\end{description}
\end{small}

These tags were used to provide knowledge about sections of the improvisation in which the participants wanted to interact or communicate directly with the system. 
Either because they felt that they wanted more explanation about how the AI was making its musical ideas or because they wanted to explain to the AI their own musical activities or intentions. 
The comments and their positional context within the improvisation timeline assisted us in understanding the aspects of the collaboration that were significant for each participant. 

...

The semi-structured interview followed a format in which participants were first asked questions to gauge their experience improvising with the system, e.g.~\textit{``what do you think about the overall experience of working with the system?''} and \textit{``did you find a balance with the system?''}.
Next, participants were asked about their experience communicating with the system during the improvisation, with general questions such as \textit{``do you think that you would like some kind of mechanisms to be able to communicate with the system?''}, as well as specific questions that referenced the participant's annotations such as \textit{``what did you want to communicate to the system at that moment?''}.

Based on the response, follow up questions were asked to probe the communication mechanisms the participant have used when improvising with another human musician (\textit{``have you improvised with a human musician before?\ldots How was it different to do it with the system from your experience?''} and \textit{``this kind of situation of being stuck in something and you wanting the other musician to respond to you. How would that work when you do it with another person?''}).

Finally, participants were asked to envision how some of these communication mechanisms could be utilised to improve communication with the system (\textit{``you have mentioned a lot about the visual cues, what kind of visual cues do you think that you could have from a system of this kind?''} and \textit{"How would you feel if the system did the same to you?"}).


participants were first asked questions to gauge their experience improvising with the system, 
their experience communicating with the system during the improvisation
follow up questions were asked to probe the communication mechanisms the participant have used when improvising with another human musician
Finally, participants were asked to envision how some of these communication mechanisms could be utilised to improve communication with the system

...


\subsection{Human interaction}

...

Understanding the way human musicians communicate with each other in an improvisational setting provides a basis for understanding the types of communication that could improve interaction with an AI musician in this setting. 

...
Communication through \textit{Musical Interaction} was mentioned consistently throughout the participant's interviews, receiving nearly twice as many references than the other codes within this theme. 
Participant's comments highlighted that musicians in an improvisational setting can communicate many different things with one another through musical interaction alone, including \textit{"key"}, \textit{"tempo"} and \textit{"tonality"}, as well as anticipation to know \textit{"what the other person is going to play"}. 
 
Analysis of participant's comments relating to \textit{Physical Interaction} when improvising with other human musicians identified that this style of communication is primarily used either when communication through the music has failed or when needing to explicitly communicate a specific piece of information that is time sensitive.
Participant P4 explained that when communicating through the music they \textit{"would present an idea and that would be so obvious"}, following on with \textit{"you might give them a dirty look, if they didn't pick up on it, but [the idea presented through the music] should be an obvious thing"}.
Participant P5 described a situation in which they would vocalise \textit{"things that are really difficult to communicate without speaking"} rather than relying on communication through the music alone; \textit{"when it comes to something complicated, sometimes it's just easier to turn around to your drummer and say... `let's go to halftime'... rather than just playing halftime and there's a whole awkward stage."}

...
In addition to the two styles of communication described above, analysis of the theme \textit{Human Interaction} also identified the importance of \textit{Past Experiences}. 
When musicians play and improvise together on a number of occasions, they start to learn aspects about the other musician's musical style that can improve their communication with one another.

Participant P1 described a situation where past musical experiences assist in their musical communication, \textit{"Because we've grown up listening to similar music, I think if I play something, that would trigger a lot of things for him and vice versa."}

...

\subsection{Understanding the system}
It is reasonable to assume that there are inherit assumptions about an `Artificial Intelligence Music System' possessing a certain level of prior musical ability, and using this phrase to describe the system in the calls for participation might have influenced the participants to expect a certain level of musical skill from the system.
Participants comments relating to the \textit{Expected musical knowledge} of the system can be grouped into two main categories: \textit{Natural - Unnatural interaction} and \textit{System being random}.
Participant P1 commented that at times the music from the system \textit{"didn't feel natural"}, explaining that \textit{"some of what the system plays sounds a bit random, not necessarily something a human would play"}.

...

Participant P1 described some of their attempts to understand the system's behaviour \textit{"if I play just basic chords, it's going to play something that's totally crazy over the top... okay, well how about I try and play something totally crazy as well and and see if [the system] wants to play chords"}.
Participant P3 described their strategies to learn how the system responds to their input \textit{"at the beginning, I wanted to show it where I wanted to go, which is basically a set of notes. ... But then I started listening back to see what [the system is] picking up? Right, to see if the system wanted to offer me something back? ... if it was going to be a pure repetition, or an analogue repetition, or randomisation of my notes, or [if the system was] going to take me somewhere else away from the set of notes that I picked".}

...

Participant P5 commented \textit{"just understanding what notes [the system] was regularly playing would help me"}.

\subsection{Structured Improvisation}

...

Participant P1 explained that they \textit{"have no idea what [the system is] going to play. There's no common ground at all to begin with"} and went on to mention \textit{"I would like if it had some kind of common ground, and I knew at least a little bit of what might come next, then I think it would be a lot more enjoyable"}.

...


Participant P2 described how improvising musicians listen and react to the musical role of the other musicians and adjust their own style accordingly, stating that \textit{"in jazz music, if someone's doing a solo, then everyone [else] stays quiet"}.
Participant P5 commented that they thought the system was \textit{"a dominating musician to play with, it just wants to keep playing its lead thing"} and identified the difficulty they experienced improvising with a system that is not aware of these musical roles, saying \textit{"there's moments where we're both sort of dominating\ldots and it sounds like a mess"}, going on to add \textit{"you can't have two dominant voices"}. 

...


The concept of the improvisation following a pre-defined structure of musical stages was mentioned by participants who expressed difficulty improvising with the system when it did not give them enough space between consecutive notes or sequences. 
Participant P4 explained that \textit{"[the system] is terrible at finding space, and it's sort of a vicious cycle"}, going on to explain that \textit{"music is about the space as well as the notes, you need silence and you need periods of very little going on. Which [the system] doesn't understand."}
Participant P3 said they \textit{"would like to be able to suggest stages"}, expressing a desire to have the ability to have a \textit{"dialogue"} with the system to \textit{"setup your set ups"} and \textit{"build up a mass of notes \ldots then let's just give each other space"}.

...

\subsection{Explicit Communication}

...

Within this theme, four key intentions that participants wished to be able to communicate to the system were identified and explored in codes \textit{signal good interaction}, \textit{signal unwanted interaction}, \textit{signal change to the system} and \textit{signal end of performance}. 
Additionally, the fifth code within this theme, \textit{system signalling to user}, explores participants desires for bi-directional communication by giving the system autonomy to signal its own desires to the human musician.

...


Participant P1 described a moment when the system played a section \textit{"that sounded so nice"} and they \textit{"would have never thought to play that"}, expressing a desire to tell the system \textit{"please do that again"} and \textit{"that was great. Go back to that. Go back to that."}

...

Giving the human musician the ability to reinforce particular musical decisions and phrases that the system produces would provide another feedback mechanism that the system could use to refine the model of musical patterns it has learned from the human musician.

...

Providing the human musician with the ability to give negative feedback to the system would add another dimension to the systems ability to refine its models of musical patterns.  
Participant P2 describes a point in their improvisation with the system where they wanted to communicate to the system \textit{``don't play the melody, don't play on top register, play in the bottom register.''}
Participant P5 describes a moment in their improvisation where they \textit{"feel this disconnect from the system"}, expressing that they \textit{"don't really know how else to communicate that what we're doing right now isn't working."}

...

Participant P5 described wanting to inform the system that they are \textit{"going to play a style of music now. Can you accompany me in that style?"}
Participant P3 described wanting to communicate moving between leading and accompanying roles with the system by communicating \textit{``okay, it's your turn, I'm going to go and do the bass lines, you go and improvise on top''}.

...


Participant P5 annotated a moment in their improvisation with the system by adding the comment \textit{``here I slow the tempo to end the piece. It would have been good if I could have notified the AI to also slow down as the song is coming to an end.''}
Participant P3 also annotated their improvisation with the system, commenting \textit{"this is where I think the system kept running past what I felt was the natural ending"}.

...


Participant P3 said that they would appreciate signals from the system as they 
\textit{``would have loved for [the system] to suggest where it wants to go''}.
Participant P5 said that the system communicating its intention before making changes would help to improve the way they improvise with the system, describing \textit{"that sort of communication, [the system] saying 'I'm going to drop down' so I know to go back up. Because obviously, if you play too much in one frequency it becomes really overwhelming there."}

...

\subsection{Implicit Communication}

...

Participant P5 annotated their improvisation recording with moments in which they had tried to communicate with the system musically, first saying \textit{"I pause here hoping that the AI will do the same so I can change the direction of the song, however realised that it just kept playing"} and at a later moment commenting \textit{"I add a bass line to try and adjust the direction of the AI, however this doesn't seem to be working, resulting in a messy sound."}

...


Participant P3 described a possible physical mechanism that could be implemented to provide an additional communication channel with the system as \textit{"some sort of body attachment, in which the system can understand that I'm looking at it \ldots or I'm looking to my instrument"}.
Participant P5 described their take on physical communication channels with the system, suggesting that communication could be \textit{"buttons, or even a verbal thing"} going on to provide an example \textit{"give me a bass harmony to this''}.
Participant P4 mentioned a communication mechanism for the system to provide visual feedback to the human musician, suggesting \textit{"if there was some way that you could just see it there, banging away, you can sort of pick out little things that it's doing in there that make sense musically"}.

...


\Section{Background}

\subsection{Explainable AI, Music and Creativity}
AI systems are increasingly improving at performing very complex and resource-demanding tasks; however, these systems usually work in isolation and have very little room for true collaboration. This limitation is particularly important for creative AI systems, since it makes it more difficult for users to interact with them in a real-time and changing environment. We need to identify mechanisms in which systems and humans can communicate with each other so that these interactions are facilitated and better outputs can be achieved. 

Recent surveys in the field of Explainable AI (XAI) have aimed at identifying the most predominant domains in which XAI is being applied. In these surveys, the field of Creative AI has been either absent \cite{Abdul:2018}, or  significantly under represented \cite{anjomshoae:aamas19}, with just a few isolated instances in the domain of game design \cite{zhu:2018,guzdial:2018}. Focused research on the role of explainability for creative AI systems has yet to be widely explored, however it is starting to grow as a new field of research. Llano et al  \cite{xcc:iccc20}, for instance, have proposed a new area of research, Explainable Computational Creativity (XCC), which not only highlights the role of explanations to describe a creative act, but also as mechanisms to make creative systems active collaborators, e.g., by adopting the notions of argumentation and advocacy. Our work presents the first study of explanations where bi-directional communication in human-machine improvisation is explored. Communication is an intrinsic element of musical improvisation, which allows those involved to establish an understanding of each other and of the direction of a performance. 


==> ResultsTable.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{|l|l|l|}
\hline
%\multicolumn{1}{|c}{\textbf{Theme}} & \multicolumn{1}{|c}{\textbf{Codes}} &\multicolumn{1}{|c|}{\textbf{Code references (\% of Theme Total)}}\\
\textbf{Theme} & \textbf{Codes} & \textbf{Code references (\% of Theme Total)}\\
\hline
\multirow{ 3}{*}{Human Interaction}         & Musical interaction & 58\% \\ 
                                            & Physical interaction & 31\%\\
                                            & Past experiences & 11\%\\
\hline
\multirow{ 3}{*}{Understanding the system}  & Expected musical knowledge & 68\% \\ 
                                            & Experimenting & 29\%\\
                                            & Understanding patterns & 3\%\\
\hline
\multirow{ 3}{*}{Structured Improvisation}  & Leading and accompanying & 67\% \\ 
                                            & Pre-performance baseline & 18\%\\
                                            & Stages during performance & 15\%\\
\hline
\multirow{ 5}{*}{Explicit Communication}    & Signal change to the system & 39\% \\ 
                                            & Signal good interaction & 22\%\\
                                            & Signal unwanted interaction & 19\% \\
                                            & Signal end of performance & 13\%\\
                                            & System signalling to user & 7\%\\
\hline
\multirow{ 2}{*}{Implicit Communication}    & Musical cue & 68\%\\ 
                                            & Physical cue & 32\%\\
\hline
\end{tabular}
\caption{Themes and codes identified through thematic analysis of participant interviews and annotations.}
\label{tab:themes}
\end{table}

\noindent\begin{table}[ht]
\centering
\begin{tabular}{|p{0.25\linewidth} | p{0.47\linewidth} c |}%{|l|l|l|}
\hline
%\multicolumn{1}{|c}{\textbf{Theme}} & \multicolumn{1}{|c}{\textbf{Codes}} &\multicolumn{1}{|c|}{\textbf{Code references (\% of Theme Total)}}\\
\textbf{Theme} & \textbf{Codes (\% of Theme Total)} \\
\hline
\multirow{ 3}{\linewidth}{Human Interaction}            & Musical interaction & (58\%)            \\ \cline{2-3}
                                                        & Physical interaction & (31\%)           \\ \cline{2-2}
                                                        & Past experiences & (11\%)               \\ \cline{2-2}
\hline
\multirow{ 3}{\linewidth}{Understanding the system}     & Expected musical knowledge & (68\%)     \\ \cline{2-2}
                                                        & Experimenting & (29\%)                  \\ \cline{2-2}
                                                        & Understanding patterns & (3\%)          \\ \cline{2-2}
\hline
\multirow{ 3}{\linewidth}{Structured Improvisation}     & Leading and accompanying & (67\%)       \\ \cline{2-2}
                                                        & Pre-performance baseline & (18\%)       \\ \cline{2-2}
                                                        & Stages during performance & (15\%)      \\ \cline{2-2}
\hline
\multirow{ 5}{\linewidth}{Explicit Communication}       & Signal change to the system & (39\%)    \\ \cline{2-2}
                                                        & Signal good interaction & (22\%)        \\ \cline{2-2}
                                                        & Signal unwanted interaction & (19\%)    \\ \cline{2-2}
                                                        & Signal end of performance & (13\%)      \\ \cline{2-2}
                                                        & System signalling to user & (7\%)       \\ \cline{2-2}
\hline
\multirow{ 2}{\linewidth}{Implicit Communication}       & Musical cue & (68\%)                    \\ \cline{2-2}
                                                        & Physical cue & (32\%)                   \\ \cline{2-2}
\hline
\end{tabular}
\caption{Themes and codes identified through thematic analysis of participant interviews and annotations.}
\label{tab:themes}
\end{table}

==> design-guidelines.tex <==
\section{Explainable interactions for human-machine improvisations}

In the previous section we have presented a detailed description of our findings from the thematic analysis. In this section, we will distil these findings into a set of design considerations for explainable AI systems. 
%
Though we are specifically looking at human machine music improvisation, we propose these design considerations could apply to other creative domains in which sustained interactions are required throughout the creative process.
%
We propose it is also the case that future AI systems in non-creative domains will also benefit from moment to moment explanations throughout the process and not just to elucidate the final outcome. 
We have ordered the following list of design considerations according to when each interaction would occur in a typical improvisation. 

\begin{description}

\item[Structure the interaction in advance:] Participants highlighted the need to have a more structured or guided interaction with the system in this study. 
Facilitating a dialog between the human and machine co-creators, to agree on structural aspects of the improvisation before commencing, would help both creative partners to reach an understanding of each other.
Specifically, three aspects related to this were:
\begin{itemize}
    \item \textit{Agreement on an initial set up:} Participants stated the need to establish a common ground with the system before beginning a performance, agreeing on musical parameters such as: the style of music (e.g. blues, jazz), whether to play in high tempo or low tempo, loud, soft, etc. 
    \item \textit{Having a structure that develops over time:} Participants expressed a desire to locate themselves and the AI within a structured process. This involves building up the performance, knowing when to move between musical stages, understanding when to give space to each other, and communicating when to end the performance. 
    \item \textit{Understand and specify the roles in music:} 
    Participants expressed difficulty improvising with a system that did not have any prior musical knowledge and hence was not aware of it's own musical role in relation to the role of it's partner. To overcome this would involve agreeing on the structures of the roles before the performance, as well as communicating the intention to move between these roles during the performance. 
\end{itemize} 
 
\item[Interrogate the system's capabilities and limitations:] This can be thought of as a practice phase where users will work with an AI system to understand what it can do and how well it can do it. Providing participants with the opportunity to interact  with any new AI system in this way is an important design consideration highlighted in \cite{amershi:2019}.
Participants in our study expressed not just the need to understand manifest behaviours which occured during the interrogation phase, but also aspects of the underlying mechanisms of the system, such as its approach to generating music (the model's decision processes) and which musical concepts it understands (e.g. chords, tempo, harmony, melody).
Understanding the systems capabilities from the outset would help users approach musical interactions with the system by setting up their expectations about how the interaction can develop.

\item[Expose the system's state during performance:] Participants expressed a desire for the system to disclose information about its current state to help them predict future behaviours. They stressed the importance of communicating upcoming musical actions and high-level musical intentions (such as ending the performance). In improvisation and creative domains in general, innovation is often driven by unpredictability and serendipitous moments. Taking this into account, the creative capability of a system should not be compromised in order to make it predictable for the user, but any unpredictability should still lead to a coherent experience. 

%This typically occurs in the middle of the interaction.
\item[Enable implicit communication:] Participants highlighted the importance of implicitly communicating intentions through the music that they play. This nuanced style of communication is an intrinsic element of co-creation in an improvisational setting.  
Providing communication mechanisms to facilitate this form of interaction would help build understanding and trust between human and AI partners.

\item[Enable explicit communication:] In any performative musical context there will be visual and (less frequently) vocal gestures. Explicit communication in real-time could be achieved through further controls, visualisations and audio/video gesture recognition. Additionally, this type of communication offers a lot of possibilities for the system and users to gather information that can enhance their mental models of each other. However, an important point to emphasise is the need for these opportunities to enable a dialogue instead of acting as control mechanisms for the user to steer the system in a specific direction. 
\end{description}







==> feedback_from_ijcai.tex <==
Review
Mark d'Inverno
Wed 20/04/2022 13:52

    Submissions

    Help Center
    Select Your Role : 
    Author 
    IJCAIarts2022 
    Mark d'Inverno 

 Print
View Reviews
Paper ID
82
Paper Title
Teaching AI-creativity through contemporary machine learning
Reviewer #1
Questions

    1. Please briefly summarize the main contributions of the paper in your own words. (Please do not include your evaluation of the paper here).
        This paper describes a course targeted to non-engineers about applying artificial intelligence and machine learning to music creation.
    2. Please discuss strengths and weaknesses of the paper along the dimensions novelty, soundness, significance and impact, relevance to AI and the arts or creativity, clarity of exposition, and credibility with regard to reproducibility.
        Project-based learning is a really powerful approach to teaching. Students are motivated by opportunities to apply what they are learning. I like how the proposed course applies that approach to learning about AI/ML in music making. Students have to produce a song using these tools. The paper describes specific modern systems used in the course, and wrapping these in the online teaching platform. 

        A weakness to the paper is a lack of analysis in the implementation of the course. It appears to be in the planning stages, and so the paper has no feedback from the students or teachers. Another weakness is that the paper lacks discussion of evaluating students. What evidence is collected to gauge how well a student meets the intended learning outcomes of the course?
    3. What opportunities are there to improve the paper? (Note that there will be no possibility for re-submission and re-evaluation in this Special Track.)
        See above. I think this course could benefit with a discussion of working methodologies on the part of artists collaborating. There's notions of curation in week 6, but some elucidation of the criteria for curation could be useful. There's also an opportunity to explore how these collaborations differ from human collaborations.
    4. Overall assessment. 
        Weak accept. Useful. A good paper. The results and insights will benefit the field. I believe it should be accepted.

Reviewer #2
Questions

    1. Please briefly summarize the main contributions of the paper in your own words. (Please do not include your evaluation of the paper here).
        This paper focusses on teaching AI creativity. More specifically, it described the design rationale behind a creative AI segment in a BSc level course on AI. They motivate the need to teach AI primarily as means to overcome challenges associated with the deductive approach of teaching AI more generally. Along with their other course materials, the describe a pop song generator as case-study system for the students to develop, exemplifying the process of putting together a complex ML pipeline by chaining together existing (pre-trained) components.
    2. Please discuss strengths and weaknesses of the paper along the dimensions novelty, soundness, significance and impact, relevance to AI and the arts or creativity, clarity of exposition, and credibility with regard to reproducibility.
        The paper is highly relevant to educators and the special track. Best practices on teaching AI creativity are relatively novel, albeit similar work has been published e.g. on best practices in teaching computational creativity (which is not references, see weaknesses). I consider it a particular strength that the paper addresses the development of an online course, on Coursera as a specific platform. The authors facilitating quite stunning solutions to complex issues, e.g. setting up "a virtualised Linux environment that provided a browser based IDE (Visual Studio Code) and a terminal". Overall, the paper is well written. 


        Major weaknesses:
        -The introduction does not identify a research gap. It clearly points out challenges in teaching creative AI - but it doesn't highlight the contribution of this specific educational paper w.r.t to the state-of-the-art on research into teaching creative AI (have others e.g. addressed similar or different, related challenges through different means?). This lowers the apparent significance of the paper. 
        -Related: the background chapter is mostly concerned with teaching AI more generally, and only briefly touches on creative AI. You say "If we filter the background work to that concerning creative applications of AI, our brief survey only revealed Fiebrink’s paper", but it looks as if you had missed out on important material. I urge the authors to take two steps: 1) Please disambiguate how your teaching goals compare to the goals in existing courses, e.g. in "creative computing" or "creative AI". For specific courses, consider e.g. Creative Computing at UAL/London (Fiebrink, Grierson), Goldsmiths/Hong Kong University of Science and Technology (Papatheodorou), Computational Creativity at Queen Mary (Colton and others), AI for Media, Arts & Design at Aalto University (Hämäläinen, Guckelsberger: https://github.com/PerttuHamalainen/MediaAI), Neural Aesthetic at NYU (https://ml4a.github.io/classes/itp-F18/). If there are strong similarities, e.g. to creative AI, I'd like to see a comparison of the teaching approaches. 2) It would be nice to see this complemented with ideas for teaching CC, which is typically more theoretical and less practice-oriented. For the difference consult: Colton, S., Pease, A., Corneli, J., Cook, M., Hepworth, R. and Ventura, D., 2015. Stakeholder groups in computational creativity research and practice. In Computational creativity research: towards creative machines (pp. 3-36). Atlantis Press, Paris. For CC teaching approaches, check out: ACKERMAN, M., Goel, A., JOHNSON, C., Jordanous, A., León, C., Perez y Perez, R., Toivonen, H. and Ventura, D., 2017. Teaching computational creativity. ICCC. Also consider checking EvoMusArt for relevant publications. I believe these steps are fundamental to highlight the significance of this work to a specific target group.
        -The background chapter seeks to motivate the teaching of creative AI based on the challenges of teaching AI more generally, but I think the argument here could be made a lot shorter, and supported but further requirements (e.g. industry and student demand) and opportunities in teaching creative AI (e.g. fun, motivation, more intuitive appeal than traditional AI applications, etc.). There is a real opportunity there to highlight why it's worthwhile to include AI creativity in university curricula, but I think it's only partially realised. 
        -The teaching goals in the case study section are not clearly laid out, but it almost seems that the system was conceived ad-hoc, with its usefulness towards various teaching goals being justified afterwards. E.g. what techniques to teach, what methods, in which form (self-taught, exercises, classroom), to cater for which base-level and variety of expertise, and to complement which other contents in the same course? This is not exactly gold-standard, and it should be discussed and reflected on critically. If this is how it usually goes in course design, that's fine, but it should be made explicit.
        -For reproducibility, it would be it would be really nice to see in the course structure table how each part was supported through the various learning activities, and how much time students were expected to spend on each of them on average. 
        -To support reproducibility further, I'd have loved to see e.g. one session to be described in more detail, with documentation of all materials / learning materials. There is still plenty of spare space for that in the manuscript.
        -The authors claim that they "identify barriers which prevent
        access and understanding of these systems" but this part of the contribution is really weak. There's only few barriers mentioned, and they have not been assessed through controlled experiments with students. I'd like to see this contribution less emphasised. In future work, I'd be really thrilled to see as part of future work how students cope with the course design, and how the course design is iterated in response. This would also provide a great opportunity for a qualitative study of student experience as the authors already point out. I would be really interested to hear about what methodology they have in mind, given that the course will run online.

        Minor issues: 
        -Some typos, grammatical mistakes, and missing words. E.g. missing full stop in abstract: "activities The". Or in background "Guzdial and Riedly" -> "Riedel". And capitalisation, e.g. "openAI’s". Missing words e.g. in Conclusion: "In the we".
        -"another trend is the use of pre-designed and sometimes pre-trained models." - I wouldn't call this a trend, as the idea has been around for a long time. E.g. as described in the design of Simon Colton's "The Painting Fool" or in the following, seminal paper:Colton, S. and Wiggins, G.A., 2012, August. Computational creativity: The final frontier?. In Ecai (Vol. 12, pp. 21-26).
        -The research aim "To consider the design of an AI-creativity system" is too fuzzy. What did you actually aim to achieve here? To identify? To build?
        -First quote of Fiebrink, 2019 is missing a reference. 
        -"We also provided students with a GPT-2 model we had fine-tuned with a dataset of Eurovision song contest lyrics." -> Unclear: is this also the Huggingface GPT-2 implementation? 
        -It's confusing that the case-study is on CS students, while the introduction particularly relates to the difficulty of teaching Creative AI to non-CS students. 
    3. What opportunities are there to improve the paper? (Note that there will be no possibility for re-submission and re-evaluation in this Special Track.)
        See advice provided in previous tab. In coarse terms, the paper would benefit from (i) stronger motivation (to assess novelty); (ii) stronger background w.r.t. existing publications on teaching creative AI and related disciplines (to assess relevance for certain teachers); (iii) more detail on the teaching material (for increased reproducibility). 

        If this was a purely scientific paper, I could not possible accept it. However, I believe it provides some really valuable practical advice, which could be improved significantly if the suggestions above were realised. I think that the submission timeframe is sufficient for that. Hence, I suggest "weak accept" and hope that the authors will follow the recommendations for revision.
    4. Overall assessment. 
        Weak accept. Useful. A good paper. The results and insights will benefit the field. I believe it should be accepted.

Reviewer #3
Questions

    1. Please briefly summarize the main contributions of the paper in your own words. (Please do not include your evaluation of the paper here).
        The paper describes the design of an online course in AI for creativity based on a song generator (music, lyrics, and synthesis). The paper describes the component of the song generator and the whole design of the course. 
    2. Please discuss strengths and weaknesses of the paper along the dimensions novelty, soundness, significance and impact, relevance to AI and the arts or creativity, clarity of exposition, and credibility with regard to reproducibility.
        the paper is novel and interesting. The main weakness is that it looks more like a progress report than an actual paper. For instance it is not clear how the initial goals have been met (or not?). Arguably, designing a course is not a well defined task, but one may wonder wwhat the reader can learn from such a report.
    3. What opportunities are there to improve the paper? (Note that there will be no possibility for re-submission and re-evaluation in this Special Track.)
        none
    4. Overall assessment. 
        Borderline Accept. Marginally above the acceptance threshold. Technically correct, but not particularly exciting or inspiring. Could be accepted more or less in its currrent form. Not a big loss if it is not included in the program.

Reviewer #4
Questions

    1. Please briefly summarize the main contributions of the paper in your own words. (Please do not include your evaluation of the paper here).
        The paper describes the design and setup of a new (novel) hands-on course on what the authors call "AI-creativity". This could be a very useful pedagogical project and a role model for other courses in the area of AI.
    2. Please discuss strengths and weaknesses of the paper along the dimensions novelty, soundness, significance and impact, relevance to AI and the arts or creativity, clarity of exposition, and credibility with regard to reproducibility.
        The paper describes the design and setup of a new (novel) hands-on course on what the authors call "AI-creativity". This could be a very useful pedagogical project and a role model for other courses in the area of AI.

        However, I feel that all this is far too preliminary for an IJCAI publication. The submitted paper describes the rationale, the fundamental ideas, and the design of the course, and the three technological components used and set up (GPT-2 for lyrics generation; Music-VAE for musical arrangement generation, DiffSinger for synthesising singing voice). However, there is no evaluation of how well this concept works, how it is/was received by the students, whether the students really found this useful and instructive, or even if the teaching materials/systems themselves (music generation systems etc.) were good enough for the task (are they in any way capable of generating outputs that are interesting and musically valuable?)

        I would very much like to see a full paper, later, with (if only preliminary) results and evaluations of well-specified questions regarding the efficacy of this teaching approach and the suitability of the chosen AI-creativity technologies. The authors themselves write "It is common for the literature to report current teaching practice, as opposed to carefully evaluating it"; unfortunately, this paper also fails to provide any careful empirical evaluation. (There would have been a full page left within the 6 page space limit.)


    3. What opportunities are there to improve the paper? (Note that there will be no possibility for re-submission and re-evaluation in this Special Track.)
        As mentioned above, I believe this is a worthwhile and interesting effort. I wish the authors much success with the couree and would love to see a paper on this, with a systematic evaluation of course and student feedback, after the first year course year, perhaps in an upcoming ICCC conference.
    4. Overall assessment. 
        Clear Reject. Unclear contribution. Needs to be reworked and/or major revision. I vote and will argue for rejection.

Go Back
© 2022 Microsoft Corporation About CMT | Docs | Terms of Use | Privacy & Cookies | Request Free SiteTwitter logo
YesNo


